Offline to Online Learning for Real-Time Bandwidth Estimation

Real-time video applications require accurate bandwidth estimation (BWE) to maintain user experience across varying network conditions. However, increasing network heterogeneity challenges general-purpose BWE algorithms, necessitating solutions that adapt to end-user environments. While widely adopted, heuristic-based methods are difficult to individualize without extensive domain expertise. Conversely, online reinforcement learning (RL) offers ease of customization but neglects prior domain expertise and suffers from sample inefficiency. Thus, we present Merlin, an imitation learning-based solution that replaces the manual parameter tuning of heuristic-based methods with data-driven updates to streamline end-user personalization. Our key insight is that transforming heuristic-based BWE algorithms into neural networks facilitates data-driven personalization. Merlin utilizes Behavioral Cloning to efficiently learn from offline telemetry logs, capturing heuristic policies without live network interactions. The cloned policy can then be seamlessly tailored to end user network conditions through online finetuning. In real intercontinental videoconferencing calls, Merlin matches our heuristic's policy with no statistically significant differences in user quality of experience (QoE). Finetuning Merlin's control policy to end-user environments enables QoE improvements of up to 7.8% compared to the heuristic policy. Lastly, our IL-based design performs competitively with current state-of-the-art online RL techniques but converges with 80% fewer videoconferencing samples, facilitating practical end-user personalization.

==> bwe.tex <==
\begin{figure*}[t!]
%\vspace{-10mm}
\centering
\begin{subfigure}[t]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth, trim={0 12cm 0 8cm}, clip]{"./figs/bw_mos_figs/overshoot_mos".PDF}
\caption{Bandwidth Overshooting.}
\label{fig:overshoot-mos}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth, trim={0 12cm 0 8cm}, clip]{"./figs/bw_mos_figs/tracking_mos".PDF}
\caption{Bandwidth Tracking.}
\label{fig:tracking-mos}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth, trim={0 13.5cm 0 6cm}, clip]{"./figs/bw_mos_figs/undershoot_mos".PDF}
\caption{Bandwidth Undershooting.}
\label{fig:undershoot-mos}
\end{subfigure}

\caption{Quality of Bandwidth Estimates vs. User Experience (MOS).}
\label{fig:undershoot-overshoot}
\vspace{-5mm}
\end{figure*}

\vspace{-2mm}
\section{Bandwidth Estimates vs. User Experience}
\label{sec:bwe}
To illustrate the importance of BWE, we conducted a preliminary study on the impact of bandwidth estimates on user QoE during RTC videoconferencing. We benchmark three bandwidth estimators: our expert UKF model, an overshooter, and an undershooter. We conduct approximately $100$ live videoconferencing calls on real networks and report the predicted video mean opinion score (MOS). Based on previous crowd sourced data, the predicted video MOS exhibits high correlation with the subjective video MOS, a gold standard metric for gauging user QoE~\cite{video-mos}. The predicted video MOS ranges from one to five with one corresponding to low QoE and five mapping to high QoE.%\NEW{The video MOS is approximated with a pretrained MOS estimator which exhibited $99\%$ correlation with user visual experience .} 
We report a subset of our findings from network environments with stable $1$ Mbps links in Figure~\ref{fig:undershoot-overshoot}. 

In Figure~\ref{fig:overshoot-mos}, the bandwidth estimator overshoots the $1$ Mbps limit, which causes the video MOS to severely degrade, oscillating between $0.0$ and $2.0$ (a MOS of $0$ indicates an error, i.e., no video frames are received). The poor bandwidth estimates severely degrade objective QoE and cause the sender to flood the network with packets, resulting in increased queuing delays and packet loss. In contrast to overshooting, in Figure~\ref{fig:undershoot-mos}, the bandwidth estimator severely underestimates the $1$ Mbps link. Although not as harsh as overshooting, the video MOS degrades due to a lack of high-quality video frames, resulting in a stable MOS of $2.0$. Specifically, the video codec leverages the bandwidth estimates to choose an encoding rate for each frame. By underestimating the available bandwidth, the video frames are encoded at a reduced bitrate to meet bandwidth requirements, delivering lower-quality video streams to the receiver. However, since the network is not congested, packets are still able to flow freely and arrive at the receiver without being lost, leading to better user experience and a higher MOS than in the overshoot case. 


Lastly, we observe the best video MOS when the bandwidth estimator tracks the bandwidth closely as demonstrated by our UKF expert in Figure~\ref{fig:tracking-mos}. By providing accurate resource estimates, packets are able to flow freely without being dropped; additionally, video frames can be encoded at higher bitrates due to the increase in estimated network resources. The increased video encoding rate translates to higher-quality video streams being delivered to the receiver which results in a stable MOS of $3.0$. In comparison to undershooting and overshooting, tracking the available bandwidth closely leads to a significant boost in objective QoE. We report the results on simple stable cases to illustrate the impact of bandwidth estimates; however, BWE becomes more challenging in live environments due to the partial observability and non-stationary nature of real networks~\cite{rl-cc-datacenter-sigmetrics}. Thus, in this work, we seek to tackle complex environments. We conduct several videoconferencing experiments on live inter-continental links in section~\ref{sec:eval}, and demonstrate that we can preserve user QoE through high-quality BWE via purely offline IL.
